Almost Tight Hardness of Approximation for $0$-Extension

In the $0$-Extension problem, we are given an undirected graph $G=(V,E)$ with non-negative edge weights $w: E\rightarrow \mathbb{R}_{\geq 0}$, a collection $T \subseteq V$ of $k$ terminals, and a metric $D$ over terminals $T$. The goal is to find a retraction $f:V\rightarrow T$ that maps every terminal to itself, while minimizing the sum over all edges of the product of the edge's weight and the distance in $D$ between the terminals to which its endpoints are assigned, i.e., \[ \sum_{\{u,v\}\in E} w_{\{u,v\}} \cdot D(f(u), f(v)). \] Fakcharoenphol, Harrelson, Rao, and Talwar achieve the best known approximation ratio of $O(\log k / \log \log k)$, while the known approximation hardness is $\Omega(\sqrt{\log k})$ assuming the unique games conjecture. In this work, we establish an $\Omega(\log^{1-\varepsilon}k)$ hardness of approximation for every constant $\varepsilon\in (0,1)$ and arbitrarily large fixed $k$, almost matching the upper bound in the exponent of $\log k$. The main technical contribution is an $\Omega(\log^{1-\varepsilon}k)$ integrality gap for the earthmover relaxation. Our construction is inspired by randomized extensions of expanders introduced by Schwartz and Tur for the metric relaxation. The result then follows from an existing theorem by Manokaran, Naor, Raghavendra, and Schwartz that translates the integrality gap for the earthmover relaxation to the approximation hardness for every fixed $k$.

==> Fig/3-ext.tex <==
% Reusable TikZ figure: two randomized extensions of the same H.
% Required: \usepackage{tikz,amsmath}
%           \usetikzlibrary{arrows.meta,calc}
% H is the supplied four-cycle plus one diagonal.
% The middle panel draws all 16 vertices and all 40 edges of Ext(H,H).
% The right panel groups the 64 vertices of Ext(Ext(H,H),H) into the
% four fibers of the projection to the original H. Each fiber induces
% a realization of Ext(H,H), indicated by the label inside its cloud.
% Shaded bands denote the matchings between these groups, not complete
% bipartite graphs. Each band represents 16 matching edges; their
% individual endpoints and the internal edges of each cloud are suppressed.
% The four labels Ext(H,H) need not denote identical matching realizations.
% No pruning is performed. Crossings without dots are not vertices.
%
% Suggested caption:
% Two successive randomized extensions using the same graph H. The first
% extension is shown explicitly. In the second extension, each cloud
% represents a realization of Ext(H,H), and shaded bands represent the
% matchings between clouds corresponding to edges of the original H.

\begingroup
\definecolor{matchingblue}{RGB}{31,109,189}
\definecolor{matchingpurple}{RGB}{126,72,166}
\definecolor{labelgray}{RGB}{75,79,85}
\begin{tikzpicture}[
  x=1cm,y=1cm,font=\small,
  fine/.style={black,line width=.40pt},
  blue matching/.style={matchingblue,line width=.36pt,opacity=.76},
  purple matching/.style={matchingpurple,line width=.32pt,opacity=.48},
  core outline/.style={black!45,line width=.35pt},
  group outline/.style={black!40,line width=.40pt,dashed,rounded corners=9pt},
  operation/.style={-{Stealth[length=2.2mm]},black!60,line width=.65pt},
  stage/.style={font=\normalsize,align=center},
  explanation/.style={text=labelgray,font=\footnotesize,align=center}
]

\newcommand{\iteratedcorecoords}[5]{%
  \coordinate (#1-center) at (#2,#3);
  \foreach \vertex/\xsign/\ysign in {2/-1/1,0/1/1,3/-1/-1,1/1/-1}{%
    \coordinate (#1-\vertex) at ({#2+#4*\xsign},{#3+#5*\ysign});
  }%
}
\newcommand{\iteratedcoreedges}[2]{%
  \foreach \edgea/\edgeb in {2/0,0/1,1/3,3/2,2/1}{%
    \draw[fine] (#1-\edgea)--(#1-\edgeb);
  }%
  \foreach \vertex in {0,...,3}{\fill (#1-\vertex) circle[radius=#2];}%
}

% Stage titles.
\node[stage] at (0,2.65) {$H$};
\node[stage] at (4.15,2.65) {$\operatorname{\widehat{Ext}}(H,H)$};
\node[stage] at (10.5,2.65) {$\operatorname{\widehat{Ext}}(\operatorname{\widehat{Ext}}(H,H),H)$};

% Input H.
\iteratedcorecoords{base}{0}{0}{.43}{.34}
\iteratedcoreedges{base}{1.45pt}
\node[above left=2pt] at (base-2) {$a$};
\node[above right=2pt] at (base-0) {$b$};
\node[below left=2pt] at (base-3) {$c$};
\node[below right=2pt] at (base-1) {$d$};

% Each arrow denotes another application of Ext(.,H).
\draw[operation] (1.0,0)--(1.85,0);
\node[explanation] at (1.43,.43) {};
\draw[operation] (6.45,0)--(7.65,0);
\node[explanation] at (7.05,.43) {};

% Coordinates for the four cores of the first extension.
\iteratedcorecoords{first-2}{2.900}{1.250}{.25}{.21}
\iteratedcorecoords{first-0}{5.400}{1.250}{.25}{.21}
\iteratedcorecoords{first-3}{2.900}{-1.250}{.25}{.21}
\iteratedcorecoords{first-1}{5.400}{-1.250}{.25}{.21}

% The five independent perfect matchings of the first extension.
% Matching over base edge {a,b}.
\draw[blue matching] (first-2-0) .. controls (3.9999,1.4186) and (4.8332,1.2786) .. (first-0-1);
\draw[blue matching] (first-2-1) .. controls (3.8167,1.1400) and (4.4833,1.1400) .. (first-0-3);
\draw[blue matching] (first-2-2) .. controls (3.6500,1.6300) and (4.6500,1.6300) .. (first-0-0);
\draw[blue matching] (first-2-3) .. controls (3.4668,1.2786) and (4.3001,1.4186) .. (first-0-2);
% Matching over base edge {b,d}.
\draw[blue matching] (first-0-0) .. controls (5.3853,0.6463) and (5.2186,-0.1871) .. (first-1-2);
\draw[blue matching] (first-0-1) .. controls (5.7500,0.3467) and (5.7500,-0.3467) .. (first-1-0);
\draw[blue matching] (first-0-2) .. controls (5.3200,0.4867) and (5.4305,-0.4867) .. (first-1-3);
\draw[blue matching] (first-0-3) .. controls (5.2186,0.1871) and (5.3853,-0.6463) .. (first-1-1);
% Matching over base edge {d,c}.
\draw[blue matching] (first-1-0) .. controls (4.8332,-1.2786) and (3.9999,-1.4186) .. (first-3-1);
\draw[blue matching] (first-1-1) .. controls (4.6500,-1.6300) and (3.6500,-1.6300) .. (first-3-3);
\draw[blue matching] (first-1-2) .. controls (4.4833,-1.1400) and (3.8167,-1.1400) .. (first-3-0);
\draw[blue matching] (first-1-3) .. controls (4.3001,-1.4186) and (3.4668,-1.2786) .. (first-3-2);
% Matching over base edge {c,a}.
\draw[blue matching] (first-3-0) .. controls (2.9800,-0.2067) and (2.9800,0.6267) .. (first-2-0);
\draw[blue matching] (first-3-1) .. controls (2.9800,-0.6267) and (2.9800,0.2067) .. (first-2-1);
\draw[blue matching] (first-3-2) .. controls (2.4800,-0.2067) and (2.4800,0.6267) .. (first-2-2);
\draw[blue matching] (first-3-3) .. controls (2.4800,-0.6267) and (2.4800,0.2067) .. (first-2-3);
% Matching over base edge {a,d}.
\draw[blue matching] (first-2-0) .. controls (3.8948,0.6891) and (4.5614,-0.1442) .. (first-1-2);
\draw[blue matching] (first-2-1) .. controls (4.0540,0.2774) and (4.8874,-0.5560) .. (first-1-1);
\draw[blue matching] (first-2-2) .. controls (3.7588,0.7573) and (4.7588,-0.0761) .. (first-1-0);
\draw[blue matching] (first-2-3) .. controls (3.5540,0.2774) and (4.3874,-0.5560) .. (first-1-3);
\draw[core outline] (first-2-center) ellipse[x radius=.51cm,y radius=.55cm];
\iteratedcoreedges{first-2}{1.05pt}
\node[fill=white,inner sep=1pt] at ($(first-2-center)+(0,0.67)$) {$H_{a}$};
\draw[core outline] (first-0-center) ellipse[x radius=.51cm,y radius=.55cm];
\iteratedcoreedges{first-0}{1.05pt}
\node[fill=white,inner sep=1pt] at ($(first-0-center)+(0,0.67)$) {$H_{b}$};
\draw[core outline] (first-3-center) ellipse[x radius=.51cm,y radius=.55cm];
\iteratedcoreedges{first-3}{1.05pt}
\node[fill=white,inner sep=1pt] at ($(first-3-center)+(0,-0.67)$) {$H_{c}$};
\draw[core outline] (first-1-center) ellipse[x radius=.51cm,y radius=.55cm];
\iteratedcoreedges{first-1}{1.05pt}
\node[fill=white,inner sep=1pt] at ($(first-1-center)+(0,-0.67)$) {$H_{d}$};

% The second extension is shown at the level of its four large clouds.
\coordinate (last-a) at (8.90,1.25);
\coordinate (last-b) at (12.10,1.25);
\coordinate (last-c) at (8.90,-1.25);
\coordinate (last-d) at (12.10,-1.25);

% Shaded bands follow exactly the five edges of H.
% Draw them first, so each band disappears underneath its endpoint clouds.
\newcommand{\extensionband}[3]{%
  \fill[matchingpurple!22]
    ($(#1)+({#3+90}:.19)$)--($(#2)+({#3+90}:.19)$)--
    ($(#2)+({#3-90}:.19)$)--($(#1)+({#3-90}:.19)$)--cycle;
}
\extensionband{last-a}{last-b}{0}
\extensionband{last-b}{last-d}{-90}
\extensionband{last-d}{last-c}{180}
\extensionband{last-c}{last-a}{90}
\extensionband{last-a}{last-d}{-38}

\foreach \cloud in {a,b,c,d}{%
  \draw[fill=white,draw=black!55,line width=.5pt]
    (last-\cloud) ellipse[x radius=.98cm,y radius=.72cm];
  \node[font=\small] at (last-\cloud) {$\operatorname{\widehat{Ext}}(H,H)$};
}

% Legend: the shaded bands summarize matchings, not dense bipartite graphs.

\draw[fine] (1.00,-2.65)--(1.45,-2.65);
\node[anchor=west] at (1.55,-2.65) {edges of $0$-clouds};
\draw[blue matching,opacity=1] (5.35,-2.65)--(5.80,-2.65);
\node[anchor=west] at (5.90,-2.65) { edges of $1$-clouds};
\fill[matchingpurple!22] (9.75,-2.75) rectangle (10.25,-2.55);
\node[anchor=west] at (10.35,-2.65) {edges of $2$-clouds};

\end{tikzpicture}
\endgroup


==> Fig/adj-levels.tex <==
% Adjacent-level analysis figure. Palette matches the t=2 instance figure.
% Native TikZ keeps the schematic editable and sharp at any magnification.
\begingroup
\definecolor{fineblue}{RGB}{32,76,113}
\definecolor{coarseblue}{RGB}{36,124,160}
\definecolor{terminalred}{RGB}{174,68,54}
\begin{tikzpicture}[
  x=1cm,y=1cm,draw=fineblue,text=fineblue,
  every node/.style={font=\small,inner sep=2pt},
  edge/.style={draw=fineblue!70,line width=.55pt},
  vertex/.style={circle,draw=fineblue,fill=white,inner sep=0pt,minimum size=4pt},
  active/.style={circle,draw=fineblue,fill=fineblue,inner sep=0pt,minimum size=4pt},
  coarse/.style={circle,draw=coarseblue,fill=white,inner sep=0pt,minimum size=7pt},
  heavy/.style={circle,draw=coarseblue,fill=coarseblue,inner sep=0pt,minimum size=7pt},
  panel/.style={draw=fineblue!35,rounded corners=5pt,line width=.5pt},
  group/.style={draw=coarseblue,densely dotted,rounded corners=8pt,line width=.9pt,fill=coarseblue!5},
  arrow/.style={-{Stealth[length=4pt]},draw=coarseblue,line width=.65pt},
  virtual/.style={draw=terminalred,dashed,line width=.7pt}
]
\path[use as bounding box] (0,0) rectangle (15.8,13.4);

% (a) Fine and coarse levels, with one possible heavy-core partition part.
\draw[panel] (0,6.6) rectangle (15.8,13.4);
\node[anchor=west,font=\small\bfseries] at (.3,13.03)
  {(a) Partition heavy cores through the adjacent coarser level};
\node[anchor=west] at (.35,11.7) {$X_j$};
\node[anchor=west,align=center] at (.25,8.86) {$X_{j-1}$};
\draw[group] (2.15,11.23) rectangle (7.4,12.18);
\node[font=\footnotesize] at (4.78,12.53)
  {one part of $R$: diameter $\leq\Lambda/4$};
\foreach \a/\b in {2.9/6.65,6.65/10.4,10.4/14.15}{
  \draw[draw=coarseblue,line width=.65pt] (\a,11.7)--(\b,11.7);
}
\node[heavy,label={[font=\footnotesize]below:$u$}] at (2.9,11.7) {};
\node[heavy,label={[font=\footnotesize]below:$v$}] at (6.65,11.7) {};
\node[coarse] at (10.4,11.7) {};
\node[coarse] at (14.15,11.7) {};
\node[font=\footnotesize] at (12.27,12.32) {other core};

\draw[group] (1.62,7.73) rectangle (7.94,9.97);
\foreach \x in {2.9,6.65}{
  \draw[draw=fineblue,fill=terminalred!9,line width=.75pt]
    (\x,8.86) ellipse (1.05 and .76);
  \draw[arrow] (\x,9.68)--(\x,11.05);
}
\foreach \x in {10.4,14.15}{
  \draw[draw=fineblue!65,fill=white] (\x,8.86) ellipse (1.05 and .76);
  \draw[arrow] (\x,9.68)--(\x,11.05);
}
\node[font=\footnotesize,fill=white] at (4.8,10.63) {$p$: contract each core};
\draw[arrow] (1.4,11.54)--(1.4,10.18);
\node[anchor=east,font=\footnotesize,align=center] at (1.35,10.75) {lifting};

% Internal edges are schematic; filled fine vertices denote membership in U.
\foreach \x in {2.9,6.65,10.4,14.15}{
  \begin{scope}[shift={(\x,8.86)}]
    \draw[edge] (-.65,.15)--(-.15,.43)--(.55,.22)--(.6,-.3)--(-.13,-.43)--(-.65,.15);
    \draw[edge] (-.15,.43)--(-.13,-.43) (-.65,.15)--(.55,.22);
    \foreach \a/\b in {-.65/.15,-.15/.43,.55/.22,.6/-.3,-.13/-.43}{
      \node[vertex] at (\a,\b) {};
    }
  \end{scope}
}
\foreach \x in {2.9,6.65}{
  \foreach \a/\b in {-.65/.15,-.15/.43,.55/.22,.6/-.3,-.13/-.43}{
    \node[active] at ({\x+\a},{8.86+\b}) {};
  }
}
\foreach \x in {10.4,14.15}{
  \node[active] at ({\x-.65},9.01) {};
}
\foreach \a/\b in {2.9/6.65,6.65/10.4,10.4/14.15}{
  \draw[edge] ({\a+.55},9.08)--({\b-.65},9.01);
  \draw[edge] ({\a+.6},8.56)--({\b-.13},8.43);
}
\node[font=\footnotesize] at (2.9,8.02) {$H_u\subset A$};
\node[font=\footnotesize] at (6.65,8.02) {$H_v\subset A$};
\node[font=\footnotesize] at (12.27,7.95) {nonheavy cores};
\node[font=\footnotesize,align=center] at (4.78,7.14)
  {lifting of $A$ has diameter $\leq\Lambda/2$\\ cores have diameter $O_t(\sigma_{j-1})\ll\Lambda$};
\node[font=\footnotesize,align=center] at (12.15,7.14)
  {filled vertices: points of $U$};

% (b) Forest and virtual metric edge on A.
\draw[panel] (0,0) rectangle (7.7,6.25);
\node[anchor=west,font=\small\bfseries] at (.3,5.87) {(b) Sample a forest};
\node[align=center,font=\footnotesize] at (3.85,5.18)
  {Delete edges with both endpoints in $A$.\\Sample $F$ from the remaining graph $G$.};
\draw[draw=terminalred!60,fill=terminalred!8,rounded corners=5pt]
  (1.05,.99) rectangle (6.65,1.75);
\node[anchor=west,font=\footnotesize,text=terminalred] at (1.14,1.37) {$A$};
\draw[edge] (2,1.37)--(2,2.39)--(1.35,3.35)--(.9,4.1);
\draw[edge] (2,2.39)--(3,3.35)--(3.5,4.1);
\draw[edge] (5.8,1.37)--(5.8,2.39)--(5.15,3.35)--(4.7,4.1);
\draw[edge] (5.8,2.39)--(6.7,3.35)--(7,4.1);
\draw[virtual] (2,1.37)--(5.8,1.37);
\node[font=\footnotesize,fill=terminalred!8,text=terminalred] at (3.9,1.37) {$d_Y(a,b)$};
\foreach \x/\y in {2/2.39,1.35/3.35,.9/4.1,3/3.35,3.5/4.1,5.8/2.39,5.15/3.35,4.7/4.1,6.7/3.35,7/4.1}{
  \node[vertex] at (\x,\y) {};
}
\node[active,draw=terminalred,fill=terminalred,label={[font=\footnotesize,text=terminalred]below:$a$}] at (2,1.37) {};
\node[active,draw=terminalred,fill=terminalred,label={[font=\footnotesize,text=terminalred]below:$b$}] at (5.8,1.37) {};
\node[font=\footnotesize,align=center] at (3.85,.48)
  {Dashed: the metric clique on $A$.\\Edge omission probability: $O_t(1/\log n)$.};

% (c) One possible extension of the same partition of A to the forest.
\draw[panel] (8.05,0) rectangle (15.8,6.25);
\node[anchor=west,font=\small\bfseries] at (8.35,5.87) {(c) Glue the partitions};
\node[align=center,font=\footnotesize] at (11.92,5.18)
  {A random shift chooses where to cut.\\Dotted outlines show possible final parts.};
\begin{scope}[shift={(8.08,0)}]
  \draw[group] (1.47,1.02) rectangle (6.32,2.78);
  \draw[group] (.54,3.02) rectangle (1.73,4.46);
  \draw[group] (2.65,3.02) rectangle (3.87,4.46);
  \draw[group] (4.34,3.02) rectangle (5.52,4.46);
  \draw[group] (6.34,3.02) rectangle (7.35,4.46);
  \draw[edge] (2,1.37)--(2,2.39)--(1.35,3.35)--(.9,4.1);
  \draw[edge] (2,2.39)--(3,3.35)--(3.5,4.1);
  \draw[edge] (5.8,1.37)--(5.8,2.39)--(5.15,3.35)--(4.7,4.1);
  \draw[edge] (5.8,2.39)--(6.7,3.35)--(7,4.1);
  \draw[virtual] (2,1.37)--(5.8,1.37);
  \foreach \x/\y in {2/2.39,1.35/3.35,.9/4.1,3/3.35,3.5/4.1,5.8/2.39,5.15/3.35,4.7/4.1,6.7/3.35,7/4.1}{
    \node[vertex] at (\x,\y) {};
  }
  \node[active,draw=terminalred,fill=terminalred] at (2,1.37) {};
  \node[active,draw=terminalred,fill=terminalred] at (5.8,1.37) {};
  \node[font=\footnotesize,align=center] at (3.9,1.97) {one part of $A$\\plus near vertices};
\end{scope}
\node[font=\footnotesize,align=center] at (11.92,.48)
  {Every final part has diameter $\leq\Lambda$ in $Y$.};
\end{tikzpicture}
\endgroup


==> Fig/expander-tower.tex <==
% Reusable TikZ figure: cloud hierarchy in the expander tower.
% Required in the paper preamble:
% \usepackage{tikz,amsmath,graphicx}
% \usetikzlibrary{arrows.meta,calc,backgrounds}
%
% This picture follows nested vertex sets in X, not the sequence X_t,...,X_1.
% The t-cloud is V(X), a j-cloud has n^j vertices and n children, a 1-cloud
% is an intact copy of H, and a 0-cloud is a single vertex.
% The first transition displays four (t-1)-clouds with matching background
% colors in the parent and expanded views. Matching edges connect them.
% Later transitions follow one nested chain. Only a few children,
% vertices, and matching edges are drawn.
% Small internal graphs stand for the further structure inside each child.
%
% To include in a paper:
% \begin{figure}[t]
%   \centering
%   \resizebox{\textwidth}{!}{\input{randomized_extension_figure.tex}}
%   \caption{The cloud hierarchy of the expander tower, from the unique
%   t-cloud V(X) to a single-vertex 0-cloud. Every j-cloud consists of n
%   disjoint (j-1)-clouds. The first transition displays four children
%   with corresponding background colors and matching edges between them.
%   The later arrows follow one nested chain, with intermediate levels
%   omitted. A 1-cloud is a copy of H. Only a few children, vertices,
%   and edges are shown.}
%   \label{fig:expander-tower-clouds}
% \end{figure}

\begingroup
\definecolor{towerblue}{RGB}{31,109,189}
\definecolor{towerpurple}{RGB}{126,72,166}
\definecolor{towergray}{RGB}{85,89,94}
\definecolor{cloudone}{RGB}{219,236,250}
\definecolor{cloudtwo}{RGB}{221,240,226}
\definecolor{cloudthree}{RGB}{252,232,207}
\definecolor{cloudfour}{RGB}{237,225,246}

\begin{tikzpicture}[
  x=1cm,y=1cm,
  font=\small,
  fine/.style={black,line width=.42pt},
  matching/.style={towerpurple,line width=.42pt,opacity=.70},
  boundary/.style={black!65,line width=.42pt},
  child boundary/.style={black!50,line width=.42pt},
  chosen/.style={towerblue,line width=.42pt},
  zoom/.style={-{Stealth[length=2mm]},towerblue,line width=.42pt},
  stage/.style={font=\normalsize,align=center},
  explanation/.style={text=towergray,align=center}
]

% The fine graph H is a four-cycle plus one diagonal.
% The coordinates can be scaled for the schematic contents of a child.
\newcommand{\towerHcoordinates}[4]{%
  \foreach \vertex/\dx/\dy in {
      0/1/1,1/1/-1,2/-1/1,3/-1/-1}{%
    \coordinate (#1-\vertex) at ({#2+#4*\dx},{#3+.8*#4*\dy});
  }%
}
\newcommand{\towerdrawH}[2]{%
  \foreach \edgea/\edgeb in {2/0,0/1,1/3,3/2,2/1}{%
    \draw[fine] (#1-\edgea)--(#1-\edgeb);
  }%
  \foreach \vertex in {0,...,3}{\fill (#1-\vertex) circle[radius=#2];}
}

% A generic parent cloud with four displayed children standing for n.
% All four children reappear in the next stage with the same colors.
\newcommand{\towercloud}[2]{%
  \coordinate (#1-center) at (#2,0);
  \foreach \i/\xx/\yy in {0/-.80/0,1/0/.65,2/.80/0,3/0/-.65}{%
    \coordinate (#1-child\i) at ({#2+\xx},\yy);
    \towerHcoordinates{#1-c\i}{#2+\xx}{\yy}{.14}
  }%
  \foreach \i/\cloudfill in
      {0/cloudone,1/cloudtwo,2/cloudthree,3/cloudfour}{%
    \fill[\cloudfill] (#1-child\i)
      ellipse[x radius=.36cm,y radius=.34cm];
  }%
  % A few lifted matching edges between the displayed child clouds.
  % These lines end at vertices, rather than at the cloud boundaries.
  \foreach \i/\j in {0/1,1/2,2/3,3/0,1/3}{%
    \draw[matching] (#1-c\i-0)--(#1-c\j-2);
    \draw[matching] (#1-c\i-1)--(#1-c\j-3);
  }%
  \foreach \i in {0,...,3}{%
    \draw[child boundary] (#1-child\i)
      ellipse[x radius=.36cm,y radius=.34cm];
  }%
  \foreach \i in {0,...,3}{\towerdrawH{#1-c\i}{.8pt}}
  \draw[boundary] (#1-center)
    ellipse[x radius=1.43cm,y radius=1.18cm];
}

% Stage 1: the entire vertex set of the final graph X.
\node[stage] at (0,1.70) {$t$-cloud};
\towercloud{top}{0}
\node[explanation] at (0,-1.65) {$n^t$ vertices};
%\node[explanation] at (0,-2.02) {$V(X)$};

% Stage 2: display all four colored (t-1)-clouds separately.
% Their cyclic order and the matching endpoints agree with the t-cloud.
\node[stage] at (4.20,1.70) { $(t-1)$-clouds};
\foreach \i/\xx/\yy in {0/-1.20/0,1/0/.87,2/1.20/0,3/0/-.87}{%
  \coordinate (next-child\i) at ({4.20+\xx},\yy);
  \towerHcoordinates{next-c\i}{4.20+\xx}{\yy}{.24}
}
\foreach \i/\cloudfill in
    {0/cloudone,1/cloudtwo,2/cloudthree,3/cloudfour}{%
  \fill[\cloudfill] (next-child\i)
    ellipse[x radius=.53cm,y radius=.45cm];
}
% A few matching edges connect vertices in different child clouds.
\foreach \i/\j in {0/1,1/2,2/3,3/0,1/3}{%
  \draw[matching] (next-c\i-0)--(next-c\j-2);
  \draw[matching] (next-c\i-1)--(next-c\j-3);
}
\foreach \i in {0,1,3}{%
  \draw[child boundary] (next-child\i)
    ellipse[x radius=.53cm,y radius=.45cm];
}
\draw[chosen] (next-child2)
  ellipse[x radius=.53cm,y radius=.45cm];
\foreach \i in {0,...,3}{\towerdrawH{next-c\i}{1pt}}
\node[explanation] at (4.20,-1.65) {$n^{t-1}$ vertices each};
\draw[zoom] (1.55,0)--(2.34,0);

% Omitted intermediate cloud levels.
\draw[zoom] (5.93,0)--(6.34,0);
\node[font=\Large] at (6.77,0) {$\cdots$};
\draw[zoom] (7.20,0)--(8.05,0);

% A 1-cloud is a copy of H. Its children are individual vertices.
\node[stage] at (9.00,1.70) {$1$-cloud};
\coordinate (one-center) at (9.00,0);
\towerHcoordinates{one}{9.00}{0}{.48}
\fill[towerblue!9] (one-0) circle[radius=3.2pt];
\draw[boundary] (one-center)
  ellipse[x radius=.95cm,y radius=.85cm];
\towerdrawH{one}{1.3pt}
\draw[chosen] (one-0) circle[radius=3.2pt];
\node[explanation] at (9.00,-1.65) {$n$ vertices};
\node[explanation] at (9.00,-2.02) {a copy of $H$};

% The final selected child is a singleton, a 0-cloud.
\node[stage] at (12.15,1.70) {$0$-cloud};
\coordinate (singleton) at (12.15,0);
\draw[zoom] ($(one-0)+(.14,0)$)
  to[out=0,in=180] ($(singleton)+(-.15,0)$);
\node[explanation,font=\footnotesize,text=towerblue]
  at (10.83,.64) {one vertex};
\fill (singleton) circle[radius=1.5pt];
\node[below=4pt] at (singleton) {$x$};
\node[explanation] at (12.15,-1.65) {$1$ vertex};
%\node[explanation] at (12.15,-2.02) {$\{x\}$};

\end{tikzpicture}
\endgroup


==> Fig/random-ext.tex <==
% Reusable TikZ picture of a single randomized extension.
% Required in the paper preamble:
%   \usepackage{tikz,amsmath}
%   \usetikzlibrary{arrows.meta,calc}
%
% The input graphs and edge colors match the supplied figure.
% Q has edges {u,v} and {u,w}. H is the cycle 2--0--1--3--2
% plus the diagonal {2,1}. Every core is a copy of H.
% Each color shows one realization of an independent uniform random
% perfect matching. Crossings without dots are not vertices.
% This is a small schematic, not an asymptotic expander instance.
%
% Suggested use:
% \begin{figure}[t]
%   \centering
%   \input{Fig/single-randomized-extension.tex}
%   \caption{A single randomized extension. Each vertex $a$ of $Q$
%   is replaced by a copy $H_a$ of $H$. Each edge of $Q$ is replaced
%   by an independent uniform random perfect matching between the
%   corresponding copies; the colors indicate the associated edge
%   of $Q$. Black edges are the edges within each copy of $H$.}
% \end{figure}

\begingroup
\definecolor{matchingblue}{RGB}{31,109,189}
\definecolor{matchingpurple}{RGB}{126,72,166}
\definecolor{labelgray}{RGB}{75,79,85}

\begin{tikzpicture}[
  x=1cm,y=1cm,
  font=\small,
  fine/.style={black,line width=.48pt},
  match uv/.style={matchingblue,line width=.48pt,opacity=.78},
  match uw/.style={matchingpurple,line width=.48pt,opacity=.72},
  core outline/.style={black!65,line width=.5pt},
  stage/.style={font=\normalsize,align=center},
  explanation/.style={font=\small,text=labelgray,align=center},
  operation/.style={-{Stealth[length=2.2mm]},black!65,line width=.7pt}
]

% Reflect the right-hand copies, as in the supplied figure.
\newcommand{\singleextcoordinates}[4]{%
  \coordinate (#1-center) at (#2,#3);
  \foreach \vertex/\xoffset/\yoffset in {
    0/.43/.34,1/.43/-.34,2/-.43/.34,3/-.43/-.34}{%
    \coordinate (#1-\vertex) at ({#2+#4*\xoffset},{#3+\yoffset});
  }%
}
\newcommand{\singleextedges}[1]{%
  \foreach \edgea/\edgeb in {2/0,0/1,1/3,3/2,2/1}{%
    \draw[fine] (#1-\edgea)--(#1-\edgeb);
  }%
  \foreach \vertex in {0,...,3}{%
    \fill (#1-\vertex) circle[radius=1.5pt];
  }%
}
\newcommand{\singleextcore}[2]{%
  \draw[core outline] (#1-center) ellipse[x radius=.73cm,y radius=.85cm];
  \singleextedges{#1}
  \node[fill=white,inner sep=1.5pt] at ($(#1-center)+(0,.99)$) {$#2$};
}

% Input H: four vertices and five edges.
\node[stage] at (.65,2.65) {Input graphs};
\singleextcoordinates{inputH}{.65}{1.15}{1}
\singleextedges{inputH}
\node at (-.15,1.15) {$H$};

% Input Q: the two colors correspond to the two output matchings.
\coordinate (Qu) at (.05,-1.35);
\coordinate (Qv) at (1.17,-.75);
\coordinate (Qw) at (1.17,-1.95);
\draw[match uv,opacity=1] (Qu)--(Qv);
\draw[match uw,opacity=1] (Qu)--(Qw);
\foreach \vertex in {u,v,w}{\fill (Q\vertex) circle[radius=1.7pt];}
\node[below=4pt] at (Qu) {$u$};
\node[right=3pt] at (Qv) {$v$};
\node[right=3pt] at (Qw) {$w$};
\node at (-.37,-1.35) {$Q$};

\draw[operation] (1.88,0)--(2.95,0);
\node[explanation,font=\footnotesize,text width=1.65cm] at (2.42,.51)
{};
 % {randomized\\extension};

% Output: one core for each vertex of Q.
\node[stage] at (5.48,2.65) {$\operatorname{Ext}(Q,H)$};
\singleextcoordinates{extu}{3.82}{0}{1}
\singleextcoordinates{extv}{6.60}{1.25}{-1}
\singleextcoordinates{extw}{6.60}{-1.25}{-1}

% Perfect matchings: each of the four vertices occurs exactly once
% on each side of each matching.
\foreach \edgea/\edgeb in {0/0,1/1,2/3,3/2}{%
  \draw[match uv] (extu-\edgea)--(extv-\edgeb);
}
\foreach \edgea/\edgeb in {0/3,1/2,2/0,3/1}{%
  \draw[match uw] (extu-\edgea)--(extw-\edgeb);
}
\singleextcore{extu}{H_u}
\singleextcore{extv}{H_v}
\singleextcore{extw}{H_w}

% Compact legend, retaining the supplied palette and thin edge styles.
\draw[fine] (.35,-2.70)--(.78,-2.70);
\node[anchor=west] at (.88,-2.70) {inter edges};
\draw[match uv,opacity=1] (3.25,-2.65)--(3.68,-2.65);
\draw[match uw,opacity=1] (3.25,-2.75)--(3.68,-2.75);
\node[anchor=west] at (3.78,-2.70) {outer edges};

\end{tikzpicture}
\endgroup


==> Fig/single-extension.tex <==
% Reusable TikZ picture. Required in the document preamble:
% \usepackage{tikz,amsmath}
% \usetikzlibrary{arrows.meta,calc,backgrounds}
%
% This is a small schematic of the operation, not an asymptotic tower
% instance. Four displayed vertices stand in for the n vertices of H.
% The displayed four-cycle is assumed shorter than the pruning threshold.
% H is drawn as the four-cycle 2--0--1--3--2 with the diagonal 2--1.
% Only the deletions associated with C are illustrated. In the pruned
% panel, its deleted coarse edges remain visible as dashed red guides so
% that the location of C can still be seen; they are not retained edges.
%
% To include in a paper:
% \begin{figure}[t]
%   \centering
%   \resizebox{\textwidth}{!}{\input{randomized_extension_figure.tex}}
%   \caption{A randomized extension and its pruning. Each vertex of Q
%   becomes a copy of H. Each edge of Q becomes an independent uniform
%   random perfect matching between the corresponding cores. A short
%   cycle C is highlighted. Pruning removes its red coarse edges and
%   preserves its fine edges. Dashed red lines mark the deleted edges in
%   the pruned extension. The small graphs are schematic, and only the
%   deletions associated with C are illustrated.}
% \end{figure}

\begingroup
\definecolor{matchingblue}{RGB}{31,109,189}
\definecolor{matchingpurple}{RGB}{126,72,166}
\definecolor{pruningred}{RGB}{211,43,45}
\definecolor{labelgray}{RGB}{75,79,85}

\begin{tikzpicture}[
  x=1cm,y=1cm,
  font=\small,
  fine/.style={black,line width=.48pt},
  match uv/.style={matchingblue,line width=.48pt,opacity=.78},
  match uw/.style={matchingpurple,line width=.48pt,opacity=.72},
  deleted/.style={pruningred,line width=.48pt},
  pruned/.style={deleted,dash pattern=on 2.5pt off 2pt},
  core outline/.style={black!65,line width=.5pt},
  stage/.style={font=\normalsize,align=center},
  explanation/.style={font=\small,text=labelgray,align=center},
  operation/.style={-{Stealth[length=2.2mm]},black!65,line width=.7pt}
]

% Give corresponding cores identical locations before and after pruning.
% Each core is a copy of the displayed four-vertex graph H.
\newcommand{\corecoordinates}[4]{%
  \coordinate (#1-center) at (#2,#3);
  \foreach \i/\xx/\yy in {
      0/.43/.34,1/.43/-.34,2/-.43/.34,3/-.43/-.34}{%
    \coordinate (#1-\i) at ({#2+#4*\xx},{#3+\yy});
  }%
}

\newcommand{\drawcore}[2]{%
  \draw[core outline] (#1-center) ellipse[x radius=.73cm,y radius=.85cm];
  \foreach \i/\j in {2/0,0/1,1/3,3/2,2/1}{%
    \draw[fine] (#1-\i)--(#1-\j);
  }%
  \foreach \i in {0,...,3}{\fill (#1-\i) circle[radius=1.35pt];}
  \node[fill=white,inner sep=1.5pt] at ($(#1-center)+(0,.99)$) {$#2$};
}

% Input graphs, shown at the left.
\node[stage] at (.65,2.65) {Input graphs};
\corecoordinates{inputH}{.65}{1.15}{1}
\foreach \i/\j in {2/0,0/1,1/3,3/2,2/1}{%
  \draw[fine] (inputH-\i)--(inputH-\j);
}
\foreach \i in {0,...,3}{\fill (inputH-\i) circle[radius=1.5pt];}
\node at (-.15,1.15) {$H$};

\coordinate (Qu) at (.05,-1.35);
\coordinate (Qv) at (1.17,-.75);
\coordinate (Qw) at (1.17,-1.95);
\draw[match uv,opacity=1] (Qu)--(Qv);
\draw[match uw,opacity=1] (Qu)--(Qw);
\foreach \a in {u,v,w}{\fill (Q\a) circle[radius=1.7pt];}
\node[below=4pt] at (Qu) {$u$};
\node[right=3pt] at (Qv) {$v$};
\node[right=3pt] at (Qw) {$w$};
\node at (-.37,-1.35) {$Q$};

\draw[operation] (1.88,0)--(2.95,0);
\node[explanation,font=\footnotesize,text width=1.65cm] at (2.42,.51)
  {randomized\\extension};

% The unpruned extension.
\node[stage] at (5.48,2.65) {$\operatorname{Ext}(Q,H)$};
\corecoordinates{preu}{3.82}{0}{1}
\corecoordinates{prev}{6.60}{1.25}{-1}
\corecoordinates{prew}{6.60}{-1.25}{-1}

% A cycle with two fine edges and two coarse edges.
\fill[pruningred!7]
  (preu-0)--(prev-0)--(prev-1)--(preu-1)--cycle;

% One realization of each independent random perfect matching.
% The uv permutation is (0,1,3,2).
% The uw permutation is (3,2,0,1).
\foreach \i/\j in {2/3,3/2}{%
  \draw[match uv] (preu-\i)--(prev-\j);
}
\foreach \i/\j in {0/3,1/2,2/0,3/1}{%
  \draw[match uw] (preu-\i)--(prew-\j);
}
\draw[deleted] (preu-0)--(prev-0);
\draw[deleted] (preu-1)--(prev-1);
\drawcore{preu}{H_u}
\drawcore{prev}{H_v}
\drawcore{prew}{H_w}
\node[text=pruningred,fill=white,inner sep=1.5pt]
  at (5.27,.67) {$C$};

% The pruning step is unweighted: count the edges in a cycle.
\draw[operation] (7.62,0)--(9.00,0);
\node[explanation] at (8.31,.32) {prune};
\node[explanation,font=\footnotesize,text width=1.8cm] at (8.31,-.52)
  {remove red\\matching edges};

% The pruned extension: keep C visible, showing its removed coarse
% edges as dashed guides. All fine edges and other displayed coarse edges
% have the same positions and solid styles as in the previous drawing.
\node[stage] at (11.58,2.65)
  {$\widehat{\operatorname{Ext}}(Q,H)$};
\corecoordinates{postu}{9.92}{0}{1}
\corecoordinates{postv}{12.70}{1.25}{-1}
\corecoordinates{postw}{12.70}{-1.25}{-1}
\fill[pruningred!7]
  (postu-0)--(postv-0)--(postv-1)--(postu-1)--cycle;
\foreach \i/\j in {2/3,3/2}{%
  \draw[match uv] (postu-\i)--(postv-\j);
}
\foreach \i/\j in {0/3,1/2,2/0,3/1}{%
  \draw[match uw] (postu-\i)--(postw-\j);
}
\draw[pruned] (postu-0)--(postv-0);
\draw[pruned] (postu-1)--(postv-1);
\drawcore{postu}{H_u}
\drawcore{postv}{H_v}
\drawcore{postw}{H_w}
\node[text=pruningred,fill=white,inner sep=1.5pt]
  at (11.37,.67) {$C$};

\node[explanation] at (5.48,-2.48)
  {One copy of $H$ per vertex of $Q$};
\node[explanation] at (11.58,-2.48)
  {All edges in $H$ remain};

% Legend and the general pruning rule.
\draw[fine] (1.05,-3.05)--(1.48,-3.05);
\node[anchor=west] at (1.58,-3.05) {fine edges};
\draw[match uv,opacity=1] (4.00,-3.05)--(4.43,-3.05);
\draw[match uw,opacity=1] (4.00,-3.14)--(4.43,-3.14);
\node[anchor=west] at (4.53,-3.05) { matching edges};
\draw[deleted] (8.30,-3.05)--(8.73,-3.05);
\draw[pruned] (8.30,-3.14)--(8.73,-3.14);
\node[anchor=west] at (8.83,-3.05) {pruned matching edges};

\end{tikzpicture}
\endgroup

